SMART: The Stochastic Monotone Aggregated Root-Finding Algorithm

We introduce the Stochastic Monotone Aggregated Root-Finding (SMART) algorithm, a new randomized operator-splitting scheme for finding roots of finite sums of operators. These algorithms are similar to the growing class of incremental aggregated gradient algorithms, which minimize finite sums of functions; the difference is that we replace gradients of functions with black-boxes called operators, which represent subproblems to be solved during the algorithm. By replacing gradients with operators, we increase our modeling power, and we simplify the application and analysis of the resulting algorithms. The operator point of view also makes it easy to extend our algorithms to allow arbitrary sampling and updating of blocks of coordinates throughout the algorithm. Implementing and running an algorithm like this on a computing cluster can be slow if we force all computing nodes to be synched up at all times. To take better advantage of parallelism, we allow computing nodes to delay updates and break synchronization. This paper has several technical and practical contributions. We prove the weak, almost sure convergence of a new class of randomized operator-splitting schemes in separable Hilbert spaces; we prove that this class of algorithms convergences linearly in expectation when a weak regularity property holds; we highlight connections to other algorithms; and we introduce a few new algorithms for large-scale optimization.

==> section_algorithms.tex <==
\section{The Algorithm}

We develop an iterative algorithm that solves~\eqref{eq:Sroot}. The algorithm forms a sequence of points $\{x^k\}_{k \in \NN} \subseteq \cH$ that converges to a root of~\eqref{eq:Sroot}. The algorithm also keeps track of a \emph{database} of $p > 0$ points that is updated at each iteration. We denote the sequence of all databases formed throughout the algorithm by $\{(\phi^k_1, \ldots, \phi^k_p)\}_{k \in \NN}\subseteq \cH^p$. The number of points $p$ in the database is chosen by the user, and this number provides a trade off between storage and computational effort. Updating the database at every iteration can be expensive, so we introduce an IID sequence of $\{0, 1\}$-valued random variables $\{\epsilon_k\}_{k \in \NN}$ that determines if and when we update the database. If $\epsilon_k = 1$, then the database is updated at iteration $k$; otherwise, the database is left alone. The user can choose $\{\epsilon_k\}_{k \in \NN}$ however they like as long as $\rho := P(\epsilon_0 = 1) > 0$. 

Often, there is a number $n_1 \in \{0, \ldots, n\}$ and a subset of operators\footnote{If $n_1 = n$, there are no such operators} $S_{n_1+1}, \ldots, S_{n}$ such that $S_{n_1+1}(x^\ast) = \cdots =S_n(x^\ast) = 0$ for all $x^\ast \in \zer(S)$. For these operators, we do not keep track of any history: once such an operator is evaluated and the sequence $\{x^k\}_{k \in \NN}$ is updated, the operator value is thrown away. In the extreme case that $n_1 = 0$, all operators are zero at the solution,~\eqref{eq:Sroot} reduces to the common fixed-point problem, and the database $\{(\phi^k_1, \ldots, \phi^k_p)\}_{k \in \NN}\subseteq \cH^p$ is superfluous. 

Beyond the cost of updating the database, it can also be expensive to obtain $x^{k+1}$ from $x^k$ by updating all $m$ of its components, so we introduce an IID sequence of $\{0, q_1^{-1}m^{-1}\}\times\cdots \{0, q_m^{-1}m^{-1}\}$-valued random variables $\{t_{k}\}_{k \in \NN}$ that determines which components of $x^{k}$ we update at the $k$th iteration. The component-choosing variable $t_k$ is coupled with an IID sequence of $\{1, \ldots, n\}$-valued random variables $\{i_k\}_{k \in \NN}$ that determine which of the $n$ operators $S_1, \ldots, S_n$ are evaluated at the $k$th iteration. If $i_k = i$ and $t_{k,j} = 1$, then the $j$th component of $x^k$ is updated at iteration $k$ using an evaluation of $(S_i(\cdot))_j$; the other operators and component are left alone. The user can choose $\{i_k\}_{k \in \NN}$ and $\{t_k\}_{k \in \NN}$ however they like as long as $q_j := P(t_{0,j} = 1) > 0$ for all $i\in \{1, \ldots, m\}$ and $p_{ij} := P(i_0 = i | t_{0,j} \neq 0) > 0$ whenever $(S_i(\cdot))_j \not\equiv 0$.

An algorithm that solves~\eqref{eq:Sroot} might use the following 3-step process: given $x^k$ 
\begin{enumerate}
\item\label{item:algNoAsyncSample} sample $i_k, t_k,$ and $\epsilon_k$;
\item\label{item:algNoAsyncx}  get $x^{k+1}$ from $x^k$ using $\{(S_{i_k}(x^k))_{j}\mid t_{k,j} \neq 0\}$ and $(\phi_{1}^k, \ldots, \phi_{p}^k)$;
\item\label{item:algNoAsyncphi} if $\epsilon_k = 1$, get $(\phi_{1}^{k+1}, \ldots, \phi_{p}^{k+1})$ using $x^{k}$ and $(\phi_{1}^k, \ldots, \phi_{p}^k)$; Otherwise set $(\phi_{1}^{k+1}, \ldots, \phi_{p}^{k+1}) = (\phi_{1}^k, \ldots, \phi_{p}^k)$.
\end{enumerate}
After $i_k$ and $t_k$ are sampled, the inactive operators and the inactive components stall until the active ones finish Steps~\ref{item:algNoAsyncx} and~\ref{item:algNoAsyncphi}. If we have access to a parallel computing device, stalling is wasteful, so in our algorithm we let all operators work in parallel and update $x^k$ whenever they finish their work. Mathematically, we form sequences of \emph{delays}\footnote{Our delays are bounded above, though this isn't strictly necessary.} $\{d_k\}_{k \in \NN} \subseteq \{0, 1, \ldots, \tau_1\}^{m}$ and $\{e^{ij}_{k}\}_{k \in \NN} \subseteq \{0, 1, \ldots, \tau_2\}$ for $i \in \{1, \ldots, n_1\}$ and $j \in \{1, \ldots, m\}$, and we replace several instances of $x^{k}$ and $\phi_l^k$ with iterates and database elements from the past  whose coordinates were formed in the last $\tau_1$ or $\tau_2$ iterations, respectively.
The final algorithm is below:
\begin{algo}\label{alg:main}
Let $\{\lambda_k\}_{k \in \NN}$ be a sequence of stepsizes. Let $a : \{1, \ldots, n_1\} \rightarrow \{1, \ldots, p\}$ be a map that assigns the $a(i)$th database element to $i$th operator ($S_i$ with $i \leq n_1$); let $p_{a(i)} = P(a(i_0) = a(i))$. Choose $x^0\in \cH$ and $(\phi_1^0, \ldots, \phi_p^0)\in \cH^p$ arbitrarily. Then for $k \in \NN$, perform the following three steps:
\begin{enumerate}
\item If $i_k \leq n_1$, set 
$$x_j^{k+1} = \begin{cases}
x_j^k - \frac{\lambda_k}{q_jm}\left(\frac{1}{np_{ij}}(S_{i_k}(x^{k-d_k}))_j - \frac{1}{np_{ij}}(S_{i_k}(\phi_{a(i_k)}^{k-e^{i_kj}_{k}}))_j  + \frac{1}{n}\sum_{i=1}^{n_1} (S_i(\phi^{k - e^{ij}_{k}}_{a(i)}))_{j}\right) & \forall j \text{ with } t_{k,j} \neq 0; \\
x_j^k & \text{otherwise.}
\end{cases}$$
\item If $i_k > n_1$, set 
$$x_j^{k+1} = \begin{cases}
x_j^k - \frac{\lambda_k}{q_jm}\left(\frac{1}{np_{ij}}S_{i_k}(x^{k-d_k}))_j  + \frac{1}{n}\sum_{i=1}^{n_1} (S_i(\phi^{k-e^{ij}_{k}}_{a(i)}))_{j}\right)& \forall j \text{ with } t_{k,j} \neq 0; \\
x_j^k & \text{otherwise.}
\end{cases}$$
\item For $l \in \{1, \ldots, p\}$, set
$$\phi_{l}^{k+1} = \begin{cases}
\phi^{k}_{l} + \epsilon_k(x^{k-d_k} - \phi^{k}_{l}) & \text{if } l = a(i_k);\\
\phi_l^{k} & \text{otherwise.}
\end{cases} $$
\end{enumerate}
\end{algo}

The $x^{k-d_k}$ iterate in Algorithm~\ref{alg:main} can be \emph{totally synchronous}, in which case $d_{k,j} = 0$ for all $j$; 
 it can be \emph{consistent-read asynchronous}, in which case $d_{k,j} = d_{k,j'}$ for all $j$ and $j'$; 
 or it can be \emph{inconsistent-read asynchronous}, in which case $d_{k,j} \neq d_{k,j'}$ for some $j$ and $j'$. 
Totally synchronous iterates are not delayed at all, so $x^{k-d_k} = x^k$ for all $k$; consistent-read asynchronous iterates are delayed, but all of their coordinates are delayed by the same amount, so $x^{k-d_k} \in \{x^k, x^{k-1}, \ldots, x^{k-\tau_1}\}$ for all $k$; inconsistent-read asynchronous iterates are delayed, and their coordinates can be delayed by different amounts, so $x^{k-d_{k,j}}_j \in \{ x^{k}_j, x^{k-1}_j, \ldots, x^{k-\tau_1}_j\}$ for all $j$, but $x^{k-d_k}$ is not necessarily an element of $\{x^k, x^{k-1}, \ldots, x^{k-\tau_1}\}$ for all $k$.

The $\phi_{a(i)}^{k-e_{k}^{ij}}$ iterate in Algorithm~\ref{alg:main} can be totally synchronous, in which case $e^{ij}_{k} = 0$ for all $i$ and $j$; it can be consistent-read asynchronous, in which case $e_k^{ij} \in \{0, \ldots, \tau_2\}$ for all $i$ and $j$; it cannot be inconsistent-read asynchronous. 

In contrast, the $S_i(\phi^{k - e^{ij}_{k}}_{a(i)})$ operator value can be totally synchronous, in which case $e^{ij}_k = 0$ for all $i$ and $j$; it can be consistent-read asynchronous, in which case $e^{ij}_k = e^{ij'}_k$ for all $i$ and all $j$ and $j'$, but $e^{ij}_k$ is not necessarily equal to $e^{i'j}_k$ for all $i$ and $i'$;  or it can be inconsistent-read asynchronous, in which case $e^{ij}_k \neq e^{ij'}_k$ for some $i$ and some $j$ and $j'$. Totally synchronous operator values are not delayed at all, so $S_i(\phi^{k - e^{ij}_{k}}_{a(i)}) = S_i(\phi^k)$ for all $k$; consistent-read asynchronous operator values are delayed, but all of their coordinates are delayed by the same amount, so $S_i(\phi^{k - e^{ij}_{k}}_{a(i)}) \in  \{S_i(\phi^{k }_{a(i)}), \ldots, S_i(\phi^{k - \tau_2}_{a(i)})\}$ for all $k$, even if $S_i(\phi^{k - e^{ij}_{k}}_{a(i)}) \neq S_{i'}(\phi^{k - e^{i'j}_{k}}_{a(i)})$ for all $i$ and $i'$; inconsistent-read asynchronous operator values are delayed, and their coordinates can be delayed by different amounts, so $(S_i(\phi^{k - e^{ij}_{k}}_{a(i)}))_j \in  \{(S_i(\phi^{k }_{a(i)}))_j, \ldots, (S_i(\phi^{k - \tau_2}_{a(i)}))_j\}$ for all $j$, but $S_i(\phi^{k - e^{ij}_{k}}_{a(i)})$ is not necessarily an element of $\{S_i(\phi^{k - 1}_{a(i)}), \ldots, S_i(\phi^{k - \tau_2}_{a(i)})\}$ for all $k$.

The delays $\{d_k\}_{k \in \NN}$ and $\{e^{ij}_k\}_{k \in \NN}$ come with no particular order. They can induce maximal delays at all times, e.g., $d_{k,j} = \tau_1$ for all $j$ and $k$, in which case the oldest information possible is used in every iteration; they can be cyclic, e.g., $d_{k,j} = k \mod \tau_1+1$ for all $j$ and $k$, in which case the same information is used for $\tau_1$ consecutive iterations in a row, and all the intermediate information is thrown away; but in general, the delays can be arbitrary. These delays are artificially imposed, but we can also incur delays that are beyond our control. 

Uncontrolled delays can occur in the $x^{k}$ iterate when a processor, called $\text{Proc}_1$, attempts to read coordinates $x_1^k, \ldots, x_m^k$ while another processor, called $\text{Proc}_2$, attempts to replace $x^k$ with $x^{k+1}$. It can happen that $\text{Proc}_1$ successfully reads coordinate $x_1^k$ before $\text{Proc}_2$ replaces it with $x_1^{k+1}$, but that $\text{Proc}_2$ replaces $x_2^k, \ldots, x_m^{k}$ with $x_2^{k+1}, \ldots, x_m^{k+1}$ before $\text{Proc}_1$ attempts to read this group of coordinates. When $\text{Proc}_1$ finishes reading, it will have the iterate $(x_1^k, x_2^{k+1}, \ldots, x_m^{k+1})$, which is not necessarily equal to any previous iterate $x^{t}$ with $t \leq k$. This effect is exacerbated if multiple processors attempt to write and read simultaneously, but in Algorithm~\ref{alg:main}, $x^{k-d_k}$ is inconsistent-read asynchronous, so these uncontrolled delays cause no trouble. 

Inconsistent-read delays of $\phi_{a(i)}^{k-e_{k}^{ij}}$ rarely occur, but $S_i(\phi^{k - e^{ij}_{k}}_{a(i)})$ is likely to be inconsistent-read asynchronous precisely because the operator-value, not its argument, is usually stored in memory. Even when~$\phi_{a(i)}^k$ is stored in memory, it is not updated to $\phi_{a(i)}^{k+1}$ until after $S_i(\phi_{a(i)}^{k+1})\in \{S_i(\phi_{a(i)}^{k}), S_i(x^{k-d_k})\}$ has been computed, but of course, $S_{i'}(\phi_{a(i')}^{k+1})$ may still need to be computed for all $i'$ with $a(i') = a(i)$. 

In general, including inconsistent-read asynchronous iterates leads to tedious convergence proofs with many-term recursive identities and complicated stepsizes. The recursive identities are necessary to control algorithm progress in a chaotic environment. The stepsizes, on the other hand, can be be optimized and have a clear dependence on the delays, sampling probabilities, and problem data. In both the inconsistent-read and consistent-read cases, the algorithm will converge with the same range of parameters. However, the rates of convergence depend on a measure of inconsistency, which we call $\delta$
\begin{align}\label{eq:deltadef}
\delta := \sup_{\substack{k \in \NN \\ j, j' \in \{1, \ldots, m\}}} |d_{k,j} - d_{k,j'}|.
\end{align}
When $\delta = 0$, the $x^{k-d_k}$ are consistent-read asynchronous, and the convergence rates improve. Otherwise $\delta \in \{0, \ldots, \tau_1\}$ and the convergence rates degrade with increasing $\delta.$ Of course, when $\delta$ is not known explicitly, it can be replaced by its upper bound $\tau_1$.  

~\\~\\
\indent If all of the sampling variables are statistically independent and the stepsizes are chosen small enough, Algorithm~\ref{alg:main} converges:

\begin{theorem}[Convergence of Algorithm~\ref{alg:main}]\label{thm:newalgoconvergence}
For all $k \geq 0$, let $\cI_k = \sigma((i_k, t_j))$, let $\cE_k = \sigma(\varepsilon_k)$, let 
$$\cF_k := \sigma(x^0, \ldots, x^k, \phi^0, \ldots, \phi^k) = \sigma(x^0, \ldots, z^k, \phi^0),$$ and suppose that $\{ \cI_k, \cE_k, \cF_k\}$ are independent. Suppose that~\eqref{eq:coherence} holds. Finally, suppose that there are constants $\underline{\lambda}, \overline{\lambda} > 0$ such that $\{\lambda_k\}_{k\in \NN} \subseteq [\underline{\lambda}, \overline{\lambda}]$, and  
\begin{align}\label{eq:weaklambdabound}
\overline{\lambda}^2 < \begin{cases}
\min_{i,j}\left\{\frac{2\underline{\lambda} n^2p_{ij} \beta_{ij}}{\frac{3\umu_j\tau_1}{m\sqrt{\underline{q}}} + \frac{2\umu_j}{\underline{q}m}}\right\} & \text{if $n_1 = 0$}; \\
\min_{i,j}\left\{\frac{\underline{\lambda}n^2 p_{ij}\beta_{ij}}{\frac{\umu_j\tau_1}{m\sqrt{\underline{q}}}\sqrt{2(\tau_2+2)} + \frac{\umu_j(\tau_2 + 2)}{m\underline{q}}}\right\} & \text{if $n_1 > 0$}.
\end{cases}
\end{align}
Then
\begin{enumerate}
 \item \textbf{Convergence of operator values.}\label{thm:newalgoconvergence:part:operatorvalues}  For $i \in \{1, \ldots, n\}$, the sequence of $\cH$-valued random variables $\{S_i(x^{k-d_k})\}_{k \in \NN} \as$ converges strongly to $S_i(x^\ast)$.
\item \textbf{Weak convergence.} \label{thm:newalgoconvergence:part:weak} 
Suppose that $I-S$ is demiclosed. Then the sequence of $\cH$-valued random variables $\{x^k\}_{k \in \NN} \as$ weakly converges to a $\cS$-valued random variable.
\item \textbf{Linear convergence.} \label{thm:newalgoconvergence:part:linear} Let $\eta <  \min_{i} \{\rho p_{a(i)}\},$ let $\alpha \in [0, 1)$, let $\underline{q} = \min_j\{q_j\}$, let $\umu = \min_{j} \{\umu_j\}$, and let 
\begin{align}\label{eq:asynclambdalinear}
\lambda &\leq \min_{i,j}\left\{\frac{2\eta(1-\alpha)n^2p_{ij}\beta_{ij}}{\frac{2\umu_j\eta(\tau_2 + 2)}{q_jm}\left(1 + \frac{\delta\eta}{\tau_2 + 1} + \frac{5\sqrt{2(\tau_2 + 2)}\alpha^2\delta}{m\umu \left( \sqrt{2(\tau_2 + 2)} + \tau_1 \sqrt{\underline{q}} \right) }\right) + \frac{\umu_j\eta\tau_1\sqrt{2(\tau_2 + 2)}}{m\sqrt{\underline{q}}} \left(2+\frac{\eta}{1-\eta}\right) + 4\mu(\tau_2+1)\alpha(1-\alpha)n^2p_{ij}\beta_{ij}} \right\}.
\end{align}
Then if~\eqref{eq:essstrongquasimono} holds, there exists a constant $C(z^0, \phi^0) \in \vR_{\geq 0}$ depending on $x^0$ and $\phi^0$ such that for all $k \in \vN$, 
\begin{align*}
\EE\left[d_{\cS}^2(x^k)\right] &\leq  \left(1 - \frac{2\alpha\mu\lambda}{\tau_1+1} \right)^{k/(\tau_1 + 1)}\EE\left[d_\cS^2(x^0) + C(x^0, \phi^0)\right].
\end{align*}
\end{enumerate}
\end{theorem}

The proof of the Theorem~\ref{thm:newalgoconvergence} without delay (i.e., $d_k \equiv 0$ and $e^{ij}_{k}  \equiv 0$) is presented in Section~\ref{sec:nonasync}. The proof of the full theorem is in Appendix~\ref{sec:async}

